On Computing Relevant Features for Explaining NBCs

Despite the progress observed with model-agnostic explainable AI (XAI), it is the case that model-agnostic XAI can produce incorrect explanations. One alternative are the so-called formal approaches to XAI, that include PI-explanations. Unfortunately, PI-explanations also exhibit important drawbacks, the most visible of which is arguably their size. The computation of relevant features serves to trade off probabilistic precision for the number of features in an explanation. However, even for very simple classifiers, the complexity of computing sets of relevant features is prohibitive. This paper investigates the computation of relevant sets for Naive Bayes Classifiers (NBCs), and shows that, in practice, these are easy to compute. Furthermore, the experiments confirm that succinct sets of relevant features can be obtained with NBCs.

==> tabs/ex02a.tex <==
%
\begin{tabular}{|c|ccccc|c|} \toprule
  & $\prob(a)$ & $\prob(r_1|a)$ & $\prob(\neg{r_2}|a)$ & $\prob(r_3|a)$
  & $\prob(\neg{r_4}|a)$ & $\nu(a)$
  \\ \midrule
  %
  $\prob(\cdot)$ & 0.10 & 0.95 & 0.95 & 0.02 & 0.80 &
  \\
  %
  $\lprob(\cdot)$ & 1.70 & 3.95 & 3.95 & 0.09 & 3.78 & 13.47
  \\ \bottomrule
\end{tabular}


==> tabs/ex02b.tex <==
%
\begin{tabular}{|c|ccccc|c|} \toprule
  & $\prob(\neg{a})$ & $\prob(r_1|\neg{a})$ &
  $\prob(\neg{r_2}|\neg{a})$ & $\prob(r_3|\neg{a})$ &
  $\prob(\neg{r_4}|\neg{a})$ & $\nu(\neg{a})$ 
  \\ \midrule
  %
  $\prob(\cdot)$ & 0.90 & 0.03 & 0.18 & 0.34 & 0.08 &
  \\
  %
  $\lprob(\cdot)$ & 3.89 & 0.49 & 2.29 & 2.92 & 1.47 & 11.06
  \\ \bottomrule
\end{tabular}


==> tabs/ex03.tex <==
\renewcommand{\tabcolsep}{0.575em}
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{|c|cccccc||c|cccccc|} \hline
  $w_0^{\oplus}$ &
  $v^{\oplus}_{0,1}$ & $v^{\oplus}_{1,1}$ &
  $v^{\oplus}_{0,2}$ & $v^{\oplus}_{1,2}$ &
  $v^{\oplus}_{0,3}$ & $v^{\oplus}_{1,3}$ &
  %
  $w_0^{\ominus}$ &
  $v^{\ominus}_{0,1}$ & $v^{\ominus}_{1,1}$ &
  $v^{\ominus}_{0,2}$ & $v^{\ominus}_{1,2}$ &
  $v^{\ominus}_{0,3}$ & $v^{\ominus}_{1,3}$
  \\ \hline
  25 &
  15 & 15 &
  15 & 30 &
  20 & 25 &
  %
  35 &
  15 & 20 &
  20 & 10 &
  10 & 20
  \\ \hline
\end{tabular}


==> tabs/ex04.tex <==
\renewcommand{\tabcolsep}{0.425em}
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{|c|cccccccc||c|cccccccc|} \hline
  $w_0^{\oplus}$ &
  $v^{\oplus}_{0,1}$ & $v^{\oplus}_{1,1}$ &
  $v^{\oplus}_{0,2}$ & $v^{\oplus}_{1,2}$ &
  $v^{\oplus}_{0,3}$ & $v^{\oplus}_{1,3}$ &
  $v^{\oplus}_{0,4}$ & $v^{\oplus}_{1,4}$ &
  %
  $w_0^{\ominus}$ &
  $v^{\ominus}_{0,1}$ & $v^{\ominus}_{1,1}$ &
  $v^{\ominus}_{0,2}$ & $v^{\ominus}_{1,2}$ &
  $v^{\ominus}_{0,3}$ & $v^{\ominus}_{1,3}$ &
  $v^{\ominus}_{0,4}$ & $v^{\ominus}_{1,4}$
  \\ \hline
  1.70 &
  1.00 & 3.95 &
  3.95 & 1.00 &
  3.98 & 0.09 &
  3.78 & 2.39 &
  %
  3.89 &
  3.97 & 0.49 &
  2.29 & 3.80 &
  0.58 & 2.92 &
  1.47 & 3.92
  \\ \hline
\end{tabular}


==> tabs/ex06e.tex <==
\begin{table*}[tb]
  \begin{center}
    \renewcommand{\arraystretch}{1.125}
    \renewcommand{\tabcolsep}{0.5em}
    \begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}\hline
      \diagbox{$k$}{$r$} 
      & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16
      \\ \hline\hline
      %
1 & \textemdash & 0 & 1 & \textemdash & 1 & 1 & \textemdash & 1 & 1 & \textemdash & 1 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash\\
\hline
2 & \textemdash & \textemdash & 0 & 1 & \textemdash & 1 & 1 & \textemdash & 1 & 1 & \textemdash & 1 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash\\
\hline
3 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & 1 & \textemdash & 1 & \textemdash & \textemdash & \textemdash & 2 & \textemdash & 2 & \textemdash & \textemdash\\
\hline
4 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & 2 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & 4 & \textemdash\\
\hline
5 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & 6\\
\hline
      %
    \end{tabular}
    \caption{DP table for $\fml{S} = \{1, 2\}$ (Example~\ref{ex:06})} \label{tab:ex06e}
  \end{center}
\end{table*}


==> tabs/ex06g.tex <==
\begin{table*}[tb]
  \begin{center}
    \renewcommand{\arraystretch}{1.125}
    \renewcommand{\tabcolsep}{0.5em}
    \begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}\hline
      \diagbox{$k$}{$r$} 
      & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16
      \\ \hline\hline
      %
1 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & 1 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash\\
\hline
2 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & 1 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash\\
\hline
3 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & 1 & \textemdash & \textemdash\\
\hline
4 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & 1 & \textemdash\\
\hline
5 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & 1\\
\hline
      %
    \end{tabular}
    \caption{DP table for $\fml{S} = \{0, 1, 2, 3, 4, 5\}$ (Example~\ref{ex:06})} \label{tab:ex06g}
  \end{center}
\end{table*}


==> tabs/paxp-len7.tex <==
\setlength{\tabcolsep}{5pt}
\let\lpr\undefined
\let\rpr\undefined
\newcommand{\lpr}{(}
\newcommand{\rpr}{)}



\begin{table*}[t]
\centering
\resizebox{0.75\textwidth}{!}{
  \begin{tabular}{l >{\lpr}S[table-format=2,table-space-text-pre=\lpr]S[table-format=1,table-space-text-post=\rpr]<{\rpr}
  			 S[table-format=2.2] S[table-format=3]  c c c  S[table-format=1.3]  }
\toprule[1.2pt]
\multirow{2}{*}{\bf Dataset} & \multicolumn{2}{c}{\multirow{2}{*}{\bf (\#F~~~~~~\#C)}}  &  {\bf NBC}  &  & {\bf AXp}  &   \multicolumn{3}{c}{\bf PAXp}  \\
\cmidrule[0.8pt](lr{.75em}){4-4}
\cmidrule[0.8pt](lr{.75em}){6-6}
\cmidrule[0.8pt](lr{.75em}){7-9}
 & \multicolumn{2}{c}{}  & {\bf A\%} & {\bf \#I} & {\bf Length}  &  {\bf Length} & {\bf Precision} & {\bf Time} \\  

\toprule[1.2pt]

adult & 13 & 2 & 81.37 & 200 & 6.85$\pm$ 1.15 & 5.3 $\pm$ 1.13 & 98.62 $\pm$ 0.46 & 0.026 \\
\midrule
agaricus\_lepiota & 23 & 2 & 95.41 & 200 & 10.34$\pm$ 2.53 & 7.6 $\pm$ 1.45 & 97.30 $\pm$ 3.53 & 0.508 \\
\midrule
chess & 37 & 2 & 88.34 & 200 & 12.11$\pm$ 3.74 & 5.1 $\pm$ 3.80 & 82.15 $\pm$ 22.19 & 2.327 \\
\midrule
dermatology & 35 & 6 & 99.66 & 147 & 9.28$\pm$ 1.64 & 6.0 $\pm$ 1.19 & 98.40 $\pm$ 1.13 & 1.399 \\
\midrule
house-votes-84 & 17 & 2 & 89.66 & 81 & 5.31$\pm$ 1.43 & 4.3 $\pm$ 1.44 & 98.90 $\pm$ 0.32 & 0.014 \\
\midrule
kr-vs-kp & 37 & 2 & 88.07 & 200 & 12.24$\pm$ 3.85 & 5.5 $\pm$ 3.81 & 80.25 $\pm$ 24.59 & 2.553 \\
\midrule
lymphography & 19 & 4 & 88.98 & 60 & 8.82$\pm$ 0.88 & 7.4 $\pm$ 0.82 & 98.67 $\pm$ 0.45 & 0.052 \\
\midrule
mushroom & 23 & 2 & 95.51 & 200 & 10.71$\pm$ 2.33 & 7.7 $\pm$ 1.26 & 97.56 $\pm$ 2.89 & 0.481 \\
\midrule
threeOf9 & 10 & 2 & 83.13 & 103 & 4.22$\pm$ 0.42 & 4.1 $\pm$ 0.59 & 99.79 $\pm$ 0.54 & 0.002 \\
\midrule
xd6 & 10 & 2 & 81.36 & 176 & 4.55$\pm$ 0.89 & 3.8 $\pm$ 1.34 & 98.86 $\pm$ 0.70 & 0.002 \\

\bottomrule[1.2pt]
\end{tabular}
}
\caption{ Assessing PAXp explanations for NBCs. 
	%	
	Columns {\bf \#F} and  {\bf \#C} show, respectively, number of features and 
	classes in the Dataset.
	%
	 Column {\bf A\%} reports in (\%) the training accuracy of the classifier. 
	 %
	 Column {\#I} reports the number of tested instances.
	 %
	 %Column {$\delta$} reports in (\%) the used value of the parameter $\delta$.
	 %
	 Columns {\bf Length} and {\bf Precision} report, respectively, the average  
	 explanation length and the average explanation precision ($\pm$ denotes 
	 the standard  deviation). 
	 %
	 Finally, the average runtime  to compute an explanation is shown 
	 (in seconds) in {\bf Time}.
	 } 
\label{tab:paxp-len7}
\end{table*}

